Effective Attention Sheds Light On Interpretability

An attention matrix of a transformer self-attention sublayer can provably be decomposed into two components and only one of them (effective attention) contributes to the model output. This leads us to ask whether visualizing effective attention gives different conclusions than interpretation of standard attention. Using a subset of the GLUE tasks and BERT, we carry out an analysis to compare the two attention matrices, and show that their interpretations differ. Effective attention is less associated with the features related to the language modeling pretraining such as the separator token, and it has more potential to illustrate linguistic features captured by the model for solving the end-task. Given the found differences, we recommend using effective attention for studying a transformer's behavior since it is more pertinent to the model output by design.

==> figs/delimiters.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[Attention to the \septoken token.]{\includegraphics[width=\the\textwidth]{figs/AttentionSEP.pdf} }
    \qquad
    \subfloat[Attention to the \clstoken token.]{\includegraphics[width=\the\textwidth]{figs/AttentionCLS.pdf} }
    \caption{Attention scores to \septoken(top two rows) and \clstoken(bottom two rows) averaged over sequence length and dataset items for the selected GLUE task using the standard (green) and effective attention (blue).
    % \ana{Change the scale of the effective attention (from 0 to max).}
    }
    \label{fig:delimiters}
\end{figure*}


==> tables/performance.tex <==
\begin{table*}[t]
\centering
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Attention Type} & \textbf{RTE}    & \textbf{MRPC}   & \textbf{QNLI}   & \textbf{SST-2}  & \textbf{STS-B}  \\ 
\midrule
Standard       & 66.79 & 83.09 & 91.31 & 92.78 & 89.53 \\
Effective      & 66.79 & 83.09 & 91.31 & 92.78 & 89.53 \\
\bottomrule
\end{tabular}}
\caption{The GLUE subset results of the BERT-base model (trained with the standard attention) evaluated with the standard attention and the effective attention separately. Spearman correlations are reported for STS-B, and accuracy scores are reported for the remaining tasks.}
\label{tab:perf-table}
\end{table*}



